EDHOC is a New Security Handshake Standard: An Overview of Security Analysis

The paper wraps up the call for formal analysis of the new security handshake protocol EDHOC by providing an overview of the protocol as it was standardized, a summary of the formal security analyses conducted by the community, and a discussion on open venues for future work.

==> temp.tex <==
\malisa{The current presentation of the protocol is not pedagogic. Consider presenting the protocol as a diff from SIGMA-I. To do that, as a first step you need to introduce the reader to SIGMA-I. Then, add step by step additions of EDHOC.}
\paragraph{Overview}
EDHOC is a lightweight authenticated Diffie-Hellman key exchange protocol that has been developed by the IETF.
\malisa{this will be explained in the intro, consider removing the sentence}
The primary goal of EDHOC is to establish a security context for the OSCORE protocol, i.e., key material for constrained application-layer end-to-end encryption. However, it can also be used to derive keys for other applications.
\malisa{in this section, you should go straight to the point: protocol explanation. no need to do short intros again. I would propose starting the section with the following sentence on SIGMA-I.}
The cryptographic core of EDHOC is based on the MAC-then-Sign variant of the SIGMA-I protocol, a variant of the SIGMA protocol that provides identity protection against active attackers on the Initiator.
In general terms, the SIGMA protocol is a way for two parties to communicate securely over an insecure network by exchanging keys and messages that can only be understood by the intended recipients.
\malisa{previous sentence is too generic, consider removing}
Nevertheless, EDHOC introduces some modifications with respect the original SIGMA rationale to be applicable in constrained environments.
In the classical Sign-then-MAC approach described in Krawczyk et al. \cite{2003_Krawczyk}, peers send both a signature and a MAC to authenticate. Instead, in the MAC-then-Sign variant the MAC is computed first and it is sent under the signature instead of being sent explicitly.
To adapt the protocol to constrained environments, EDHOC deviates in one noticeable aspect from SIGMA: credential identifiers are non-unique.
Thus, a receiver of a signature needs to trial-verify it under possibly multiple public keys matching the sent credential identifier, making the protocol vulnerable to attacks in which adversarially-controlled public keys are among the matching ones (see Guenther et al. \cite{2023_Guenther}).
To be as compact and lightweight as possible, EDHOC involves essential components like Elliptic Curve Diffie-Hellman (ECDH) for key exchange, Concise Binary Object Representation (CBOR) data format for extremely small message formats, CBOR Object Singing and Encryption (COSE) for protecting the CBOR encoded message by means of security services like signing, MACing and encryption of CBOR-serialized data, and Constrained Application Protocol (CoAP) for message transportation.
\elsa{Should this be in the intro or here? Should I refer to the repspective RFC?}
\malisa{You cannot assume a reader is familiar with any of the terms above: COSE, CBOR, CoAP. Careful when writing such text, you either need to introduce what it is somehow or not use it all.}
The intermediate and session keys in EDHOC are obtained through  Key Derivation Functions (KDF) that use as much previous information as possible.
We will refer to this functions as $EDHOC\_KDF$.
%CBOR (Concise Binary Object Represnetation), formalized in RFC8949 \cite{CBOR} is used for compact encoding, whereas the cryptographic algorithms used in EDHOC are defined in COSE (CBOR Object Singing and Encryption), formalized in RFC8152 \cite{COSE}.
%As for CoAP, it is described in RFC 7252 and is a specialized web transfer protocol designed for use with constrained devices and low-power, low-bandwidth networks in the context of Internet of Things.
EDHOC specifies four different authentication methods, depending on whether peers use signature keys or static Diffie-Hellman keys (see Table \ref{tab:method_EDHOC}). 
When using a static Diffie-Hellman key the authentication is provided by a Message Authentication Code (MAC) computed from an ephemeral-static elliptic curve Diffie-Hellman (ECDH) shared secret. 
Otherwise, the signature provides the needed authentication.
MAC authentication allows for lower message size compared to signature authentication (100s of bytes when using static DH keys versus 200s of bytes when using signatures).


\section{Security}


Draft 00 was studied by Norrman et al. \cite{2020_Norrmana}, who present a formal analysis of all four methods in a symbolic Dolev-Yao model using the TAMARIN prover.
The Dolev-Yao model is an adversary model that employs idealized cryptographic primitives and that allows the adversary to control the communication channel and interact with protocol sessions by dropping, injecting or modifying messages.
In their analysis they also added two more adversary capabilities: long-term key reveal and ephemeral key reveal.
Their main goal was to verify properties such as session key material, entity authentication and forward secrecy.
Regarding authentication, they proved two flavors of it.
The first one is injective agreement, which guarantees to an initiator I (resp. Responder R) that whenever I (resp. R) completes a run with a Responder R (resp. Initiator I), then R (resp. I) has been engaged in the protocol as a Responder (resp. Initiator).
It also guarantees that I and R agree on a set of parameters, including the session key material.
The second variant of authentication is implicit agreement, which establishes that a party A assumes that any party B that knows the session key material must be the intended party.
In their analysis they show that implicit agreement on the session key material and the initiator's identity hold for all four authentication methods.
Contrary, given that EDHOC aims to protect the Initiator's identity, injective agreement on the initiator's identity does not hold for any of the methods.
As for the injective agreement on the session key material, it is not supported whenever the Initiator uses methods 1 or 3, i.e., static Diffie-Hellman key.
This means that different authentication methods have different authentication strengths.
To solve it, they propose to add a fourth message from R to I carrying a MAC based on a key derived from the session key material.
As for the Forward Secrecy property, they show that it is supported on all authentication methods.
They also highlight the lack of consideration of non-repudiation in the specification.
Lastly, they point out an attack due to unintended peer authentication, i.e., lack of verification of $ID\_CRED_R$ of message 2 by the Initiator.
This is because, according to the specification, parties must be configured with a policy restricting the set of peers they run EDHOC with, but the Initiator is not required to verify that the identity of the Responder is the sames as the one intended.
Their proposed solution was to make the Initiator verify whether the identity of the Responder matched the intended one.
Their proposals where studied by the LAKE Working Group and included in draft 05.

Draft 07 was studied by Kim et al. \cite{2021_Kim}. They leveraged BAN Logic (a set of rules for defining and analyzing information exchange protocols) and AVISPA (Automated Validation of Internet Security Protocols and Applications) to formally verify EDHOC protocol in both asymmetric and symmetric variants (note that the symmetric variant is no longer supported by the current version of EDHOC protocol).
Their results indicate that the protocol is vulnerable against a type of denial of service attack in which a large number of requests deplete a node's resource (resource exhaustion attack), and privacy attacks affecting the identity credentials ($ID\_CRED\_R$ and $ID\_CRED\_I$ in the asymmetric version and $ID\_PSK$ in the symmetric variant).
Even though $ID\_CRED_R$ and $ID\_CRED_I$ do not have cryptographic purpose in the protocol, they serve to retrieve the peer's public authentication keys.
Thus, an attacker can easily break the privacy of $ID\_CRED_R$ by establishing the session key with the responder, leading to a partial privacy disclosure of the responder's identity.
They recommend to include several improvements in future versions, such as to authenticate the first message and provide a way to validate the second message, while offering a solution to protect against resource exhaustion attacks.

Later on, Jacomme et al. \cite{2023_Jacomme} presented a symbolic analysis of draft 12 of EDHOC protocol in which they combined different recent developments in formal methods. 
They used SAPIC+, a tool that combines three different provers (TAMARIN, PROVERIF and DEEPSEC).
They studied all four methods, in addition to the Key Encapsulation Method (KEM) for the Quantum variant.
Their analysis confirms that even though EDHOC is resistant against basic threat models, there are still multiple weaknesses when considering more advance threat scenarios. 
Firstly, they found a flaw in the key derivation and proposed to fix it by adding a final key derivation that would depend on both $PRK\_4e3m$ and $TH\_4$.
This would have the following benefits: (1) the session key is different from the MAC key, (2) a key confirmation implies authentication of all the data, (3) a dishonest party cannot control the final value of the session key and (4) the final state of the protocol is simplified since only the session key needs to be stored, rather than storing a key and a transcript.
Secondly, they detected a Machine-in-the-Middle (MitM) type of attack where the attacker intercepts the ephemeral key shares and replaces them with the neutral element of the Diffie-Hellman group, leading to both parties having a shared secret equal to this neutral element (transcript collision attack).
The attacker can carry out the attack by using the fields $C_R$, $C_I$ or $EAD$ of unbounded length to inject chosen data.
To fix this vulnerability they proposed to alter the order of the arguments inside the hash computation (see Jacomme et al. \cite{2023_Jacomme} for details).
They also noted that the protocol could be vulnerable against downgrade attacks, event though non of the current hash functions exhibited this kind of attack.
Moreover, they detected an attack due to the possibility of resending the last message, which lead to a nonce reuse of AEAD, breaking confidentiality and integrity.
Thus, it must not be allowed when using randomized signatures.
They also detected a privacy leak when the list of trusted identities for the Initiator I is only missing I's identity.
Lastly, they highlighted cases in which non-repudiation would be unclear.
These include: (1) sessions sharing the same $PRK\_4e3m$ due to acceptance of low-order points or the identity group element and (2) signatures being malleable.
The proposals where studied by the LAKE Working Group and were included in draft 14, except for the non-repudiation cases, which were considered side cases that did not need to be detailed in the draft.

Draft 14 was later on analyzed following a code-based game playing framework by Guenther et al. \cite{2023_Guenther}.
The code-based game-playing technique aims to upper bound the advantage of an adversary in attacking some cryptographic construction, i.e., the difference between the probability that the adversary outputs 1 in two different scenarios.
Initially, the problem is represented as a code-based game, named game 0.
In the next steps, the games are sequentially modified, creating a sequence or chain of games in which the last game has the property that it cannot be won by the adversary, i.e., the advantage is zero.
By using the fundamental lemma of game playing (see Bellare et al. \cite{2004_Bellare} for details), the probability of the adversary winning the original game can be bounded.
They performed a computational cryptographic analysis of method 0 of EDHOC (both initiator and responder use signature keys).
They used a strong adversary model in which the attacker is allowed to register malicious keys with colliding identifiers.
The proposed improvements were added in further successive drafts, up until draft 17.
They proposed the use of a dedicated session key instead of reusing the last key exchange internal key for clear key separation and composable security.
This final key was already added in draft 14 $PRK\_out$), following recommendation of Jacomme et al. \cite{2023_Jacomme}.
Secondly, to strengthen EDHOC against attacks leveraging non unique credentials, they suggest including full/unique credentials in the transcript hashes ($TH\_3$ and $TH\_4$).
In addition, they propose to build transcript hashes based on plaintext rather than the ciphertext.
Finally, they suggested not to reuse keys across HKDF calls of Extract and Expand for key separation.
Even though they only studied method 0, concerns about non unique credentials are applicable as well for methods 1 and 2.

Lastly, the most recent security analysis of EDHOC was performed by Cottier et al. \cite{2022_Cottier} and refers to draft 15.
It consists of a computational proof (using code-based game-playing technique) on method 4, i.e., static Diffie-Hellman keys.
Regarding confidentiality and key privacy, they suggest replacing the empty string used as salt with $TH\_2$ in the derivation of $PRK\_2e$ to protect against salt collision attacks.
As for mutual authentication security, they detected a Key Compromise impersonation (KCI) attack on $PRK\_3e2m$. 
They suggest modifying the construction of message 3 by splitting it in two parts: (1) the first one contains the identity credentials of the initiator and is encrypted using the corresponding encryption key $sk_3$ derived from $PRK\_3e2m$, (2) the other half corresponds to the authentication tag $t\_3$ and the $EAD\_3$ and is sent without encryption.
This change has not been included in any of the drafts.
Lastly, they prove that the Responder exhibits attacks in $2^{64}$ operations, contradicting the 128-bit security level. 
The proposed fix, similar to other security analysis, is to add a fourth message in the protocol.
